CogVideoX: Text-to-Video Diffusion Models with An Expert Transformer

We present CogVideoX, a large-scale text-to-video generation model based on diffusion transformer, which can generate 10-second continuous videos aligned with text prompt, with a frame rate of 16 fps and resolution of 768 * 1360 pixels. Previous video generation models often had limited movement and short durations, and is difficult to generate videos with coherent narratives based on text. We propose several designs to address these issues. First, we propose a 3D Variational Autoencoder (VAE) to compress videos along both spatial and temporal dimensions, to improve both compression rate and video fidelity. Second, to improve the text-video alignment, we propose an expert transformer with the expert adaptive LayerNorm to facilitate the deep fusion between the two modalities. Third, by employing a progressive training and multi-resolution frame pack technique, CogVideoX is adept at producing coherent, long-duration, different shape videos characterized by significant motions. In addition, we develop an effective text-video data processing pipeline that includes various data preprocessing strategies and a video captioning method, greatly contributing to the generation quality and semantic alignment. Results show that CogVideoX demonstrates state-of-the-art performance across both multiple machine metrics and human evaluations. The model weight of both 3D Causal VAE, Video caption model and CogVideoX are publicly available at https://github.com/THUDM/CogVideo.

==> figures/caption_example1.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.9\linewidth]{images/caption_example1.jpg}
\end{center}
\end{figure}

==> figures/caption_example2.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.9\linewidth]{images/caption_example2.jpg}
\end{center}
\end{figure}

==> figures/caption_example6.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.9\linewidth]{images/caption_example6.jpg}
\end{center}
\end{figure}

==> figures/caption_example7.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.9\linewidth]{images/caption_example7.jpg}
\end{center}
\end{figure}

==> figures/v2v/v2v_1_1.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.9\linewidth]{images/v2v/v2v_1_1.png}
\end{center}
\vspace{-8mm}
\end{figure}


==> figures/v2v/v2v_1_2.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.9\linewidth]{images/v2v/v2v_1_2.png}
\end{center}
\vspace{-8mm}
\end{figure}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections-backup/abaltion.tex <==


\section{Ablation}
\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{images/ab_us.png}
        \caption{Bottom aligned}
        \label{fig:a}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{images/ab_ex.png}
        \caption{Bottom aligned}
        \label{fig:b}
    \end{subfigure}
    \begin{subfigure}[b]{0.50\textwidth}
        \includegraphics[width=\textwidth]{images/ab_rl.png}
        \caption{Bottom aligned}
        \label{fig:c}
    \end{subfigure}
    \begin{subfigure}[b]{0.46\textwidth}
        \includegraphics[width=\textwidth]{images/ab_sr.png}
        \caption{Bottom aligned}
        \label{fig:d}
    \end{subfigure}
    \caption{Overall caption for the figure.}
    \label{fig:subfigures}
\end{figure}

We conducted ablation studies on some of the designs mentioned in Section~\ref{sec:model} to verify their effectiveness.


\subsection{Position Embedding}
First, we compared 3D RoPE with sinusoidal absolute position encoding. As shown in Figure~\ref{fig:d}, the loss curve using 3D RoPE converges significantly faster than that with sinusoidal encoding.
Then we compared the use of 3D RoPE alone with the combination of 3D RoPE and learnable absolute position embedding. As shown in Figure~\ref{fig:c}, the loss curves of both methods converge almost identically. For simplicity, we chose to use 3D RoPE alone.

\subsection{Expert Adaptive Layernorm}
We experimented with different ways of incorporating experts: expert LayerNorm and MLP, and expert Layernorm only. Our experiments found that adding expert MLP does not effectively accelerate the model's convergence (Figure~\ref{fig:b}). To reduce the model parameters, we only chose to use expert adaptive Layernorm.

==> sections-backup/data.tex <==
\section{Data Process}

We collected tens of thousands of hours of videos from the internet, converting various types such as vlogs, animations, documentaries, etc. Then, we used a scene detection tool to segment long videos into single-shot clips. At the same time, we retained some clips that have scene transitions between similar shots. After that, we applied multiple filters and re-caption to all video clips.

\subsection{Video Filtering}

Due to the highly noisy distribution of video data, a significant portion is not suitable for training video generation models. Video generation models need to learn the dynamic information of the world, encompassing motion and change, with video data serving as the carrier of this dynamic information. However, videos do not necessarily equate to an accurate representation of the world's dynamics, primarily due to two reasons: first, videos are human-created, and artificial editing may distort the authentic dynamic information; second, the quality of videos can significantly drop due to issues during filming, such as camera shakes and substandard equipment.

Beyond the intrinsic quality of the videos, we also consider how well the video data supports model training. Videos with minimal dynamic information or lacking connectivity in dynamic aspects are considered detrimental. Consequently, we have developed a set of negative labels, which include:

\begin{itemize}
    \item \textbf{Editing}: Videos that have undergone obvious artificial processing, such as re-editing and special effects, causing degradation of the visual integrity.
    \item \textbf{Lack of Motion Connectivity}: Video segments with image transitions lacking motion connectivity, commonly seen in videos artificially spliced or edited from images.
    \item \textbf{Low Quality}: Poorly shot videos with unclear visuals or excessive camera shake.
    \item \textbf{Lecture Type}: Videos focusing primarily on a person continuously talking with minimal effective motion, such as educational content, lectures, and live-streamed discussions.
    \item \textbf{Text Dominated}: Videos containing a substantial amount of visible text or primarily focusing on textual content.
    \item \textbf{Noisy Screenshots}: Noisy videos recorded from phone or computer screens.
\end{itemize}

We collected 20,000 video data points and labeled each video for the presence of negative tags. Utilizing these annotations, we trained several filters based on video-llama to screen out low-quality video data.

In addition, we calculated the optical flow scores and image aesthetic scores of all training videos and dynamically adjusted the threshold rages during the training process to ensure the fluency and aesthetic quality of the generated videos. 


\subsection{Video Caption}
Typically, most video data does not come with corresponding descriptive text, so it is necessary to convert the video data into textual descriptions to provide the essential training data for text-to-video models. Currently, there are some video caption datasets available, such as Panda70M~\citep{chen2024panda}, COCO Caption~\citep{lin2014microsoft}, and WebVid~\cite{bain2021frozen}. However, the captions in these datasets are usually very short and fail to describe the video's content comprehensively. We propose a pipeline to generate video captions from image captions and then fine-tune an end-to-end video captioning model to obtain more dense video captions. Our final video captioning model can generate more detailed descriptions of videos, further enhancing the quality of video generation \citep{betker2023improving}.


\input{figures/pipeline}

\paragraph{Dense Video Caption Data Generation.} To generate high-quality video caption data, we established a complex data generation pipeline, as detailed in Figure~\ref{fig:video_caption_gen}. First, we used the Panda70M video captioning model to generate short captions for the videos. Then, we employed the image recaptioning model from CogView3~\citep{zheng2024cogview3} to create dense image captions for the frames within the videos. Subsequently, we used GPT-4 to summarize all the image captions to produce the final video caption. To accelerate the generation process from image captions to video captions, we fine-tuned a Llama 2 model~\citep{touvron2023llama} using the summary data generated by GPT-4~\citep{GPT4}, enabling large-scale video caption data generation. Additional details regarding the video caption data generation process can be found in Appendix~\ref{ap:video_caption_gen}.


\paragraph{Dense Video Caption Model Training.} To further accelerate the video caption generation process, we fine-tuned an end-to-end video understanding model, called CogVLM2-Caption, based on the CogVLM2-Video~\citep{CogVLM2-Video} and Llama 3~\citep{llama3modelcard}, using the dense caption data generated from aforementioned pipeline. We trained on 100k videos using a training cluster of 16 machines, each equipped with 8 A100 GPUs, for 10 epochs. This achieved the capability to generate dense video captions as described above through the pipeline method. Examples of video captions generated by our end-to-end model are shown in Appendix~\ref{ap:video_caption_example}. In Appendix~\ref{ap:v2v}, we also present some examples of video generation where a video is first input into CogVLM2-Caption to generate captions, which are then used as input for CogVideoX to generate new videos, effectively achieving video-to-video generation.





==> sections-backup/introduction.tex <==
\section{Introduction}

In recent years, diffusion models have made groundbreaking advancements in multimodal generation, such as image, video, speech and 3D generation. Among these, video generation is a rapidly evolving field and being extensively explored. Given the successful experiences with Large Language Models (LLMs), comprehensive scaling up of data volume, training iterations, and model size consistently enhances model performance. Additionally, there is more mature scaling experience with transformers compared to UNet. And DiT \citep{peebles2023scalable} has shown that transformers can effectively replace UNet as the backbone of diffusion models. Thus, transformer is a better choice for video generation.
However, long-term consistent video generation remains a significant challenge.  % 第一段介绍任务重要性和我们工作的亮点，例如开源。DiT的讨论不应该在这里

The first challenge is that constructing a web-scale video data pipeline is considerably more difficult than for textual data. Video data is extremely diverse in distribution, quality varies greatly, and simple rule-based filtering is often insufficient for effective data selection. Consequently, processing video data is both time-consuming and highly complex.
There are numerous meaningless unrealistic videos, such as poor-quality edits and computer screen recordings. And many videos are difficult to watch normally, such as those with excessively shaky cameras. These types of data are harmful to the generative model's ability to learn genuine dynamic information. They need to be meticulously processed and filtered out to ensure the quality of the training dataset.

Additionally, most video data available online lacks accurate textual descriptions, significantly limiting the model's ability to grasp precise semantic understanding. To address this issue, we trained a video understanding model capable of accurately describing video content. We use it to generate new textual descriptions for all video data. 
To advance the field of video generation, we have decided to open-source this description model.

The high training cost is another significant challenge. If the video is unfolded into a one-dimensional sequence in the pixel space, the length would be extraordinarily long. To keep the computational cost within a feasible range, we trained a 3D VAE that compresses the video along both spatial and temporal dimensions. Additionally,  unlike previous video models that use a 2D VAE to encode each frame separately, 3D VAE ensures continuity among frames so that the generated videos do not flicker. 

Moreover, to improve the alignment between videos and texts, we propose an expert transformer to facilitate the interaction between the two modalities. Then, to ensure the consistency of video generation and to capture large-scale motions, it is necessary to comprehensively model the video along both temporal and spatial dimensions. Therefore, we opt for 3D full attention, as detailed in Section~\ref{sec:expert-transformer}.




==> sections-backup/model.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.7\linewidth]{images/transformer.png}
\end{center}
\caption{\textbf{Our model architecture.} }
\label{fig:model}
\end{figure}

\subsection{Expert Transformer}\label{sec:expert-transformer}

\paragraph{Patchify}
After being encoded into latent vectors of shape $T \times H \times W \times C$ by the 3D causal VAE, the video latents are patchified  along the spatial dimensions, resulting sequence $z_{\text{vision}}$ of length $T\cdot \frac{H}{p} \cdot \frac{W}{p}$. 
% VAE encodes the video into a latent vector of shape $T \times H \times W \times C$. Then we patchify the latent along the spatial dimensions, generating sequence $z_{vision}$ of length $T\cdot \frac{H}{p} \cdot \frac{W}{p}$. 
We do not patchify along the temporal dimension in order to enable joint training of images and videos.

\paragraph{3D-RoPE}
Rotary Position Embedding (RoPE)~\citep{su2024roformer} is a relative positional encoding that has been demonstrated to capture inter-token relationships effectively in LLMs, particularly excelling in modeling long sequences. To adapt to video data, we extend RoPE to 3D. 
Each latent in the video tensor can be represented by a 3D coordinate $(x, y, t)$.
We independently apply 1D-RoPE to each dimension of the coordinates, each occupies $3/8$, $3/8$, $2/8$ of the hidden states's channel. The resultsing encoding are then concatenate along the channel dimension to obtain the final 3D-RoPE encoding.

\paragraph{Expert Transformer Block}
We concatenate the embeddings of both text and video at the input stage to better align visual and semantic information. However, the feature spaces of these two modalities differ significantly, and their embeddings may even have different numerical scales. To better process them within the same sequence, we employ Expert Adaptive Layernorm to handle each modality independently.
As shown in Figure~\ref{fig:model}, following DiT~\citep{peebles2023scalable}, we use the timestep $t$ of the diffusion process as the input to the modulation module. 
Then, the Vision Expert Adaptive Layernorm and Text Expert Adaptive Layernorm independently apply this modulation mechanism to the vision hidden states and text hidden states respectively. This method promotes the alignment of feature spaces across two modalities while minimizing additional parameters.



\paragraph{3D Full Attention}
Previous works \citep{singer2022make, guo2023animatediff} often employ separated spatial and temporal attention to reduce computational complexity and facilitate fine-tuning from text-to-image models. However, as illustrated in Figure~\ref{fig:attention}, this separated attention approach requires extensive implicit transmission of visual information, significantly increasing the learning complexity and making it challenging to maintain the consistency of large-movement objects. Considering the great success of long-context training in LLMs and the efficiency of FlashAttention, we propose a 3D text-video hybrid attention mechanism. This mechanism not only achieves better results but can also be easily adapted to various parallel acceleration methods. 


\begin{wrapfigure}{r}{0.5\textwidth}
\centering
\includegraphics[width=\linewidth]{images/attention.png}
\caption{The separated spatial and temporal attention makes it challenging to  handle the large motion between adjacent frames. In the figure, the head of the person in frame $i+1$ cannot directly attend to the head in the frame $i$. Instead, visual information can only be implicitly transmitted through other background patches. This can lead to inconsistency issues in the generated videos.}
\label{fig:attention}
\vspace{-10mm}
\end{wrapfigure}





==> sections-backup/pretraining.tex <==
\section{Training}

\begin{figure}[ht]
\begin{center}
\includegraphics[width=\linewidth]{images/CogVideoX.png}
\end{center}
\caption{
The diagram of Mixed duration training and Frame Pack. To fully utilize the data and enhance the model's generalization capability, we train with videos of different durations within the same batch.}
\label{fig:framepack}
\end{figure}

\subsection{Setting}
We mixed images and videos during training, treating each image as a single-frame video. Additionally, we employed progressive training from the resolution perspective. For the diffusion setting, we adopt v-prediction~\citep{salimans2022progressive} and zero SNR~\citep{lin2024common}, following the noise schedule used in LDM~\citep{rombach2022high}.
During diffusion training for timestep sampling, we also employed an explicit uniform timestep sampling method, which benefits stable training. 

\subsection{Frame Pack}
Previous video model training methods often involved jointly training images and fixed frames videos. However, this approach led to two major problems: 1. There is a significant gap between the two input types using bidirectional attention, with images having 1 frame while videos having dozens of frames. We observed that models trained this way tend to diverge into two generative modes based on the token number and do not generalize well. 2. For training with a fixed duration, we need to discard short videos and truncate long videos, which prevents full utilization of the videos of varying frames.

To address these issues, we chose mixed-duration training, which means training videos of different lengths together. However, inconsistent data shapes within the batch make training difficult. Inspired by Patch'n Pack \citep{dehghani2024patch}, we place videos of different lengths into the same batch to ensure consistent shapes within each batch, a method we refer to as Frame Pack. 

\subsection{resolution prograssive training}
Our training pipeline is divided into three stages: low-resolution training, high-resolution training, and high-quality video fine-tuning. Similar to images, internet videos also include a significant amount of low-resolution videos. Prograssive training can effectively utilize various resolution videos. 
Moreover, training at low resolution initially can equip the model with coarse-grained modeling capabilities, followed by high-resolution training to enhance the model's ability to capture fine details. Compared to direct high-resolution training, staged training can reduce the overall training time.
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.9\linewidth]{images/ive.png}
\end{center}
\caption{We compared the initial generation states of extrapolation and interpolation when increasing resolution with RoPE encoding. Extrapolation tends to generate multiple small, clear, and repetitive images, while interpolation generates a blurry large image.}
\label{fig:ive}
\end{figure}

\paragraph{Extrapolation of position code}
When adapting low-resolution position encoding to high-resolution, we consider two different methods: interpolation and extrapolation. We show the effects of two methods in Figure~\ref{fig:ive}. Interpolation tens to preserve global information more effectively, whereas the extrapolation better retains local details. Given that RoPE is a relative position encoding, We chose the extrapolation to maintain the relative position between pixels. 

\paragraph{High-Quality fine-tuning}
Since the filtered pre-training data still contains a certain proportion of dirty data, such as subtitles, watermarks, and low-bitrate videos, we selected a subset of higher quality video data, accounting for 20\% of the total dataset, for fine-tuning in the final stage. This step effectively removed generated subtitles and watermarks and slightly improved the visual quality. However, we also observed a slight degradation in the model's semantic ability.


\subsection{Explicit Uniform Sampling}
~\citet{ho2020denoising} defines the training objective of diffusion as 
\begin{equation}~\label{eq:ddpm-loss}
    L_\mathrm{simple}(\theta) := \mathbf{E}_{t, x_0, \epsilon}{ \left\| \epsilon - \epsilon_\theta(\sqrt{\bar\alpha_t} x_0 + \sqrt{1-\bar\alpha_t}\epsilon, t) \right\|^2},
\end{equation}
where $t$ is uniformly distributed between 1 and T.
The common practice is for each rank in the data parallel group to uniformly sample a value between 1 and 
T. In theory, this is equivalent to Equation~\ref{eq:ddpm-loss}. However, in practice, the results obtained from such random sampling are often not sufficiently uniform, and since the magnitude of the diffusion loss is related to the timesteps, this can lead to significant fluctuations in the loss.
$Explicit\ Uniform\ Sampling$ is to divide the range from 1 to T into n intervals, where n is the number of ranks. Each rank then uniformly samples within its respective interval. This method ensures a more uniform distribution of timesteps. As shown in Figure~\ref{fig:a}, the loss curve from training with Explicit Uniform Sampling is noticeably more stable.


==> sections-backup/results.tex <==
\section{Empirical Evaluation}
We trained a series of models of various sizes. For all subsequent evaluations, we will use the largest model (referred to as CogVideoX).
In this section, we present the experimental validation of CogVideoX through two primary methods: automated metric evaluation and human assessment, providing a thorough analysis of the performance and quality of the generated videos. 
We trained a series of models with different parameter sizes. The following evaluation defaults to using our largest model.

\subsection{Results of Automated Metric Evaluation} 

\paragraph{Baselines.} We chose several top-performing text-to-video models as our baselines for comparison, including T2V-Turbo~\citep{li2024t2v}, AnimateDiff~\citep{guo2023animatediff}, VideoCrafter2~\citep{chen2024videocrafter2}, OpenSora~\citep{opensora}, Show-1~\citep{zhang2023show}, Gen-2~\citep{gen2}, Pika~\citep{pika} and LaVie-2~\citep{wang2023lavie}.


\input{figures/evaluation_results}
\paragraph{Evaluation Metrics.} To evaluate the text-to-video generation, we employed several metrics from VBench~\citep{huang2023vbench}: \emph{Human Action}, \emph{Scene}, \emph{Dynamic Degree}, \emph{Multiple Objects}, and \emph{Appearance Style}. VBench is a suite of tools designed to automatically assess the quality of generated videos. We have selected certain metrics from VBench, excluding others that do not align with our evaluation needs. For example, the color metric, intended to measure the presence of objects corresponding to specific colors across frames in the generated video, assesses the model's quality by calculating the probability. However, this metric may mislead video generation models that exhibit greater variation, thus we chose not to include it in our evaluation. For longer-generated videos, some models might produce videos with minimal changes between frames to obtain higher scores, but these videos lack rich content. Therefore, a metric for evaluating the dynamism of the video becomes more important. To address this, we employed two video evaluation tools, We also employed the \emph{Dynamic Quality} from Devil~\citep{liao2024evaluationtexttovideogenerationmodels} and \emph{GPT4o-MTScore} from ChronoMagic~\citep{yuan2024chronomagic}, which focus more on the dynamic characteristics of videos. \emph{Dynamic Quality} is defined by the integration of various quality metrics with dynamic scores. This approach mitigates biases arising from negative correlations between video dynamics and video quality, leading to a more thorough assessment of video quality. ChronoMagic, for instance, introduces the \emph{GPT4o-MTScore}, a metric designed to measure the metamorphic amplitude of time-lapse videos, such as those depicting physical, biological, and meteorological changes. This metric is obtained by extracting frames from the generated videos at regular intervals and using GPT-4o~\citep{gpt4o} to score the degree of change, providing a fine-grained assessment of video dynamism. This method ensures a more accurate evaluation of the content's variability over time, countering the potential bias of static frame sequences in scoring.



\paragraph{Results.} Table~\ref{table:results} provides a detailed comparison of the performance of our CogVideoX model with other models. Our model achieved the best performance in 5 out of the 7 metrics and showed competitive results in the remaining 2 metrics. These results demonstrate that our model not only excels in video generation quality but also outperforms previous models in handling various complex dynamic scenes. Additionally, Figure~\ref{fig:radar} presents a radar chart comparing the performance of different models.


\begin{figure}[ht]
\begin{center}
\includegraphics[width=\linewidth]{images/t2v/goodcase1.jpg}
\end{center}
\caption{Text to video showcases. The displayed prompt will be upsampled before being fed into the model. The generated videos contain large motion and can produce various video styles.}
\label{fig:t2vgood1}
\end{figure}

\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.98\linewidth]{images/t2v/goodcase2.jpg}
\end{center}
\caption{Text to video showcases.}
\label{fig:t2vgood2}
\end{figure}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}




% \begin{table}[]

% \centering
% \setlength\tabcolsep{3pt}

% \label{sample-table}
% \small
% \vspace{-10pt}
% \caption{\textbf{Automatic Evaluation Results per Dimension.}The table presents a comparative analysis of various video models across different dimensions. It is evident from the table that, in terms of both human motion and background effects as well as the accuracy and distinctiveness of objects, CogVideoX has achieved the current SOTA level. Furthermore, CogVideoX has garnered a commendable score in the expression of dynamic qualities, a capability that serves as a more precise indicator of the intrinsic properties of video media, distinct from the static nature of photographic images.}

% \vspace{6pt}

% \begin{tabular}{cccccccc}
% \toprule
% \multirow{2}{*}{\textbf{Models} }  & \textbf{human}  & \textbf{object} &\multirow{2}{*}{\textbf{scene}}&\textbf{dynamic} &\textbf{multiple} &\textbf{spatial} &\textbf{appearance} \\
%     & \textbf{action}& \textbf{class}& & \textbf{degree} &\textbf{objects}& \textbf{relationship}&\textbf{style}  
% \\
% \midrule
% CogVideoX & 96.80\% &93.70\% & 55.44\% & 62.22\% & 70.95\% & 61.29\% & 24.44\% \\
% {LaVie-2} & 96.40\% & 97.52\%  & 49.59\% & 31.11\% & 64.88\%  & 38.68\% & 25.09\%  \\
% {T2V-Turbo}  & 95.20\%  & 93.96\%& 55.58\% & 49.17\% & 54.65\%    & 38.67\%  & 24.42\%   \\
% {Gen-2}  & 89.20\%& 90.92\%  & 48.91\%  & 18.89\% & 55.47\%    & 66.91\%   & 19.34\%  \\
% {VideoCrafter-2.0\citep{chen2024videocrafter2}} & 95.00\% & 92.55\% & 55.29\%               & 42.50\% & 40.66\% & 35.86\% & 25.13\%  \\
% {Pika Beta} & 88.00\% & 87.45\%  & 44.80\% & 37.22\% & 46.69\% & 65.65\% & 21.89\%   \\
% AnimateDiff-V2 & 92.60\% & 90.90\%  & 50.19\% & 40.83\%        & 36.88\% & 34.60\%  & 22.42\%\\
% {OpenSora V1.2}   & 85.80\% & 83.37\%& 42.47\%   & 47.22\%    & 58.41\% & 67.51\%  & 23.89\%  \\
% {Show-1} & 95.60\%  & 93.07\%  & 47.03\% & 44.44\% & 45.47\% & 53.50\%  & 23.06\%  \\
% {HiGen}  & 86.20\%  & 86.06\%  & 44.88\% & 99.17\% & 22.39\%  & 22.43\% & 24.54\% \\  
% \bottomrule
% \end{tabular}
% \end{table}



% \iffalse



% \begin{table}[ht!]
% \centering
% \caption{Evaluation results.}
% \setlength\tabcolsep{3pt}
% \label{sample-table}
% \begin{center}
% \small
% \resizebox{0.9\linewidth}{!}{
% \begin{tabular}{ccccccccc}

% \multirow{2}{*}{\textbf{Models} }  & \textbf{subject}  & \textbf{background} &\textbf{temporal} &\textbf{motion} &\textbf{dynamic} &\textbf{aesthetic} &\textbf{imaging} &\textbf{object} \\
%     & \textbf{consistency}& \textbf{consistency}& \textbf{flickering}& \textbf{smoothness} &\textbf{degree}& \textbf{quality}&\textbf{quality} & \textbf{class}
% \\ \hline 
%         CogVideoX & 94.66\% & 95.92\% & 97.47\% & 98.10\% & 62.22\% & 55.14\% & 63.62\% & 93.70\%  \\
%         LaVie-2 & 97.90\% & 98.45\% & 98.76\% & 98.42\% & 31.11\% & 67.62\% & 70.39\% & 97.52\%  \\ 
%         T2V-Turbo (VC2) & 96.28\% & 97.02\% & 97.48\% & 97.34\% & 49.17\% & 63.04\% & 72.49\% & 93.96\%  \\ 
%         Gen-2 (2023-06) & 97.61\% & 97.61\% & 99.56\% & 99.58\% & 18.89\% & 66.96\% & 67.42\% & 90.92\%  \\ 
%         VideoCrafter-2.0\citep{chen2024videocrafter2} & 96.85\% & 98.22\% & 98.41\% & 97.73\% & 42.50\% & 63.13\% & 67.22\% & 92.55\%  \\ 
%         Pika Beta (2023-06) & 96.76\% & 98.95\% & 99.77\% & 99.51\% & 37.22\% & 63.15\% & 62.33\% & 87.45\%  \\ 
%         AnimateDiff-V2 & 95.30\% & 97.68\% & 98.75\% & 97.76\% & 40.83\% & 67.16\% & 70.10\% & 90.90\%  \\ 
%         OpenSora V1.2 & 94.45\% & 97.90\% & 99.47\% & 98.20\% & 47.22\% & 56.18\% & 60.94\% & 83.37\%  \\ 
%         Show-1 & 95.53\% & 98.02\% & 99.12\% & 98.24\% & 44.44\% & 57.35\% & 58.66\% & 93.07\%  \\ 
%         HiGen & 90.07\% & 93.99\% & 93.24\% & 96.69\% & 99.17\% & 57.30\% & 63.92\% & 86.06\% \\ 
% \hline \\

% \multirow{2}{*}{\textbf{Models} }  & \textbf{multiple}  & \textbf{human} &\multirow{2}{*}{\textbf{color}} &\textbf{spatial} &\multirow{2}{*}{\textbf{scene}} &\textbf{appearance} &\textbf{temporal} &\textbf{overall} \\
%     & \textbf{objects}& \textbf{action}& & \textbf{relation} & & \textbf{style}&\textbf{style} & \textbf{consistency}
% \\ \hline 
%         CogVideoX & 70.95\% & 96.80\% & 79.75\% & 61.29\% & 55.44\% & 24.44\% & 23.69\% & 26.73\%  \\ 
%         LaVie-2 & 64.88\% & 96.40\% & 91.65\% & 38.68\% & 49.59\% & 25.09\% & 25.24\% & 27.39\%  \\ 
%         T2V-Turbo (VC2) & 54.65\% & 95.20\% & 89.90\% & 38.67\% & 55.58\% & 24.42\% & 25.51\% & 28.16\%  \\
%         Gen-2 (2023-06) & 55.47\% & 89.20\% & 89.49\% & 66.91\% & 48.91\% & 19.34\% & 24.12\% & 26.17\%  \\ 
%         VideoCrafter-2.0 & 40.66\% & 95.00\% & 92.92\% & 35.86\% & 55.29\% & 25.13\% & 25.84\% & 28.23\%  \\
%         Pika Beta (2023-06) & 46.69\% & 88.00\% & 85.31\% & 65.65\% & 44.80\% & 21.89\% & 24.44\% & 25.47\%  \\ 
%         AnimateDiff-V2 & 36.88\% & 92.60\% & 87.47\% & 34.60\% & 50.19\% & 22.42\% & 26.03\% & 27.04\%  \\ 
%         OpenSora V1.2 & 58.41\% & 85.80\% & 87.49\% & 67.51\% & 42.47\% & 23.89\% & 24.55\% & 27.07\%  \\ 
%         Show-1 & 45.47\% & 95.60\% & 86.35\% & 53.50\% & 47.03\% & 23.06\% & 25.28\% & 27.46\%  \\ 
%         HiGen & 22.39\% & 86.20\% & 86.22\% & 22.43\% & 44.88\% & 24.54\% & 25.14\% & 27.14\% \\ \hline

% \hline \\
% \end{tabular}

% }
% \end{center}
% \end{table}

% \fi






% \begin{table}[!ht]
% \centering

% \label{sample-table}
% \small
% \vspace{-10pt}
% \caption{\textbf{Automatic Evaluation Results per Dimension.}}

% \vspace{6pt}

% \resizebox{0.8\linewidth}{!}{
%     \begin{tabular}{cccc}
%         \textbf{Models} & \textbf{\Centerstack{Dynamics Range}} & \textbf{\Centerstack{Dynamics Controllability}} & \textbf{\Centerstack{Dynamics-based Quality}} \\ \hline
%         CogVideoX       & 55.7 & 71.8 & \textbf{69.5} \\ 
%         Gen-2           & 30.8 & \textbf{82.5} & 43.6 \\ 
%         Pika            & 43.2 & 72.0 & 52.1 \\ 
%         VideoCrafter2   & 34.1 & 57.0 & 43.6 \\ 
%         OpenSora        & \textbf{61.2} & 62.4 & 63.7 \\ 
%         Show-1          & 45.1 & 73.9 & 57.7 \\ 
%     \end{tabular}
% }
% \end{table}


\input{tables/evaluation_results}


\subsection{Human Evaluation}
In addition to automated scoring mechanisms, a comparative analysis between the Kling~\citep{kling} and CogVideoX was conducted using a manual scoring system. One hundred meticulously crafted prompts were used, characterized by their broad distribution, clear articulation, and well-defined conceptual scope. We randomize videos for blind evalution. A panel of evaluators assigned scores for each detail on a scale from zero to one, with the overall total score rated on a scale from zero to five, where higher scores reflect better video quality. Reasons for any score deductions were also carefully documented. The results shown in Table~\ref{table:human_eva} indicate that our model outperforms Kling in all aspects. More details are shown in \ref{sec:human_evalution}.

\input{tables/human_evaluation}



% \begin{table}[!ht]
% \centering

% \label{sample-table}
% \small
% \vspace{-10pt}
% \caption{\textbf{Automatic Evaluation Results per Dimension.}}

% \vspace{6pt}

% \resizebox{0.8\linewidth}{!}{
%     \begin{tabular}{cccc}
%         \textbf{Models} & \textbf{\Centerstack{Dynamics Range}} & \textbf{\Centerstack{Dynamics Controllability}} & \textbf{\Centerstack{Dynamics-based Quality}} \\ \hline
%         CogVideoX       & 55.7 & 71.8 & \textbf{69.5} \\ 
%         Gen-2           & 30.8 & \textbf{82.5} & 43.6 \\ 
%         Pika            & 43.2 & 72.0 & 52.1 \\ 
%         VideoCrafter2   & 34.1 & 57.0 & 43.6 \\ 
%         OpenSora        & \textbf{61.2} & 62.4 & 63.7 \\ 
%         Show-1          & 45.1 & 73.9 & 57.7 \\ 
%     \end{tabular}
% }
% \end{table}


==> sections-backup/vae.tex <==
\section{Model Architecture}\label{sec:model}

The whole process of CogVideoX is as follows: First, a \textbf{3D causal VAE} is used to compress the video into the latent space, and the latents are patchified and unfolded into a long sequence denoted as $z_{\text{vision}}$.
Simultaneously, we encode the textual input into text embeddings $z_{\text{text}}$ using T5~\citep{raffel2020exploring}. Subsequently, $z_{text}$ with $z_{vision}$ are concatenated along the sequence dimension. The concatenated embeddings are then fed into a stack of \textbf{expert transformer} blocks.
Finally, the model output are unpatchified to restore the original latent shape, which is then decoded using 3D causal VAE decoder to reconstruct the video. In this section, we illustrate the two main component, i.e. 3D causal VAE and expert transfomer in detail.

\subsection{3D Causal VAE} 

Compared to image data, videos encompass not only spatial information but also substantial temporal information, resulting orders of magnitude of times of data volumes and computational burden. To tackle such challenge, we propose to implement a video compression module based on 3D Variational Autoencoders (3D VAEs). Our 3D VAE incorporates three-dimentional convolutions to compress videos both spatially and temporally, achieving both higher compression ratio and largely-improved quality and continuity of video reconstruction compared to previous image VAEs.

\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{images/3dvae_combined.jpg}
\end{center}
\caption{(a) Model structure of 3D VAE. The architecture comprises an encoder, a decoder and a latent space regularizer, achieving a 4$\times$8$\times$8 compression from pixels to the latents. (b) Context parallel implementation on temporal causal convolution.}
\label{fig:3dvae_combined}
\end{figure}

The model structure of 3D VAE is shown in Figure~\ref{fig:3dvae_combined}(a). The architecture comprises an encoder, a decoder and a latent space regularizer. The encoder and decoder consist of four symmetrically arranged stages, respectively performing 2-times downsampling and upsampling by the interleaving of resnet block stacked stages. The first two rounds of downsampling and upsampling involves both the spatial and temporal dimensions, while the last round only samples spatially. This enables the 3D VAE to achieve a 4-times compression in the temporal dimension and an 8$\times$8 compression in the spatial dimensions. The Gaussian latent space is constrained by a Kullback-Leibler (KL) regularizer.

Following~\cite{yu2023language}, we implement temporally causal convolution, which places all the paddings at the beginning of the convolution space, as shown in Figure~\ref{fig:3dvae_combined}(b). This ensures the future information not to influence the present or past predictions. Given that processing videos with large number of frames introduces excessive GPU memory usage, we apply context parallel technique at the temporal dimension for 3D convolution to distribute computation among multiple devices. As illustrated by Figure~\ref{fig:3dvae_combined}(b), due to the causal nature of the convolution, each rank simply sends a segment of length $k-1$ to the next rank, where $k$ indicates the temporal kernel size. This results in relatively low communication overhead.

During actual implementation, we first train 3D VAE on lower resolutions and fewer frames to save computation. We observe that the encoding of larger resolution generalizes naturally, while extending number of frames to be encoded did not work as seamlessly. 
%yzy：先不写详细训练
Therefore, we conduct a two stage training process by first training on short videos and finetuning by context parallel on long videos. Both stages of training utilize a weighted combination of L2 loss, LPIPS~\citep{zhang2018unreasonable} perceptual loss and GAN loss from a 3D discriminator.
%Therefore we first train on videos of 17$\times$256$\times$256 with frame rate 8, by batch size of 128 and 800k training steps, and finetune by context parallel on videos of 129$\times$256$\times$256, by batch size of 16 and 200k steps. Both stages of training utilize a weighted combination of L2 loss, LPIPS~\citep{zhang2018unreasonable} perceptual loss and GAN loss from a 3D discriminator.


==> sections/abaltion.tex <==


We conducted ablation studies on some of the designs mentioned in Section~\ref{sec:model} to verify their effectiveness.


\subsection{Position Embedding}
First, we compared 3D RoPE with sinusoidal absolute position encoding. As shown in Figure~\ref{fig:d}, the loss curve using 3D RoPE converges significantly faster than that with sinusoidal encoding.
Then we compared the use of 3D RoPE alone with the combination of 3D RoPE and learnable absolute position embedding. As shown in Figure~\ref{fig:c}, the loss curves of both methods converge almost identically. For simplicity, we chose to use 3D RoPE alone.

\subsection{Expert Adaptive Layernorm}
We experimented with different ways of incorporating experts: expert LayerNorm and MLP, and expert Layernorm only. Our experiments found that adding expert MLP does not effectively accelerate the model's convergence (Figure~\ref{fig:b}). To reduce the model parameters, we only chose to use expert adaptive Layernorm.
